Joint$\lambda$: Orchestrating Serverless Workflows on Jointcloud FaaS Systems

Existing serverless workflow orchestration systems are predominantly designed for a single-cloud FaaS system, leading to vendor lock-in. This restricts performance optimization, cost reduction, and availability of applications. However, orchestrating serverless workflows on Jointcloud FaaS systems faces two main challenges: (1) additional overhead caused by centralized cross-cloud orchestration; and (2) a lack of reliable failover and fault-tolerant mechanisms for cross-cloud serverless workflows. To address these challenges, we propose Joint$\lambda$, a distributed runtime system designed to orchestrate serverless workflows on multiple FaaS systems without relying on a centralized orchestrator. Joint$\lambda$ introduces a compatibility layer, Backend-Shim, leveraging inter-cloud heterogeneity to optimize makespan and reduce costs with on-demand billing. By using function-side orchestration instead of centralized nodes, it enables independent function invocations and data transfers, reducing cross-cloud communication overhead. For high availability, it ensures exactly-once execution via datastores and failover mechanisms for serverless workflows on Jointcloud FaaS systems. We validate Joint$\lambda$ on two heterogeneous FaaS systems, AWS and Aliyun, with four workflows. Compared to the most advanced commercial orchestration services for single-cloud serverless workflows, Joint$\lambda$ reduces makespan by up to 3.3$\times$ while saving up to 65% in cost. Joint$\lambda$ is also up to 4.0$\times$ faster than state-of-the-art orchestrators for cross-cloud serverless workflows, while achieving competitive cost in representative scenarios and providing strong execution guarantees.

==> ref.tex <==
\begin{thebibliography}{100}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{jonas2019cloud}
E.~Jonas, J.~Schleier-Smith, V.~Sreekanti, C.-C. Tsai, A.~Khandelwal, Q.~Pu, V.~Shankar, J.~Carreira, K.~Krauth, N.~Yadwadkar \emph{et~al.}, ``Cloud programming simplified: A berkeley view on serverless computing,'' \emph{arXiv preprint arXiv:1902.03383}, 2019.

\bibitem{gao2022mrass}
F.~Gao, H.~Wang, P.~Shi, X.~Fu, T.~Zhong, and J.~Kong, ``Mrass: Dynamic task scheduling enabled high multi-cluster resource availability in jointcloud,'' in \emph{2022 IEEE International Conference on Joint Cloud Computing (JCC)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2022, pp. 43--50.

\bibitem{aws}
\BIBentryALTinterwordspacing
AWS, ``Aws lambda,'' 2024, accessed 2024.05.30. [Online]. Available: \url{https://aws.amazon.com/lambda}
\BIBentrySTDinterwordspacing

\bibitem{ali}
\BIBentryALTinterwordspacing
Aliyun, ``Aliyun function compute,'' 2024, accessed 2024.05.30. [Online]. Available: \url{https://www.aliyun.com/product/fc}
\BIBentrySTDinterwordspacing

\bibitem{lithops}
\BIBentryALTinterwordspacing
lithops cloud, ``Lithops,'' 2024, accessed 2024.05.30. [Online]. Available: \url{https://github.com/lithops-cloud/lithops}
\BIBentrySTDinterwordspacing

\bibitem{gcp}
Google, ``Google cloud functions,'' \url{https://cloud.google.com/functions}, 2024, accessed 2024.05.30.

\bibitem{googleoutage}
\BIBentryALTinterwordspacing
------, ``Google cloud accidentally deletes unisuper’s online account due to ‘unprecedented misconfiguration’,'' 2024, accessed 2024.05.30. [Online]. Available: \url{https://www.theguardian.com/australia-news/article/2024/may/09/unisuper-google-cloud-issue-account-access}
\BIBentrySTDinterwordspacing

\bibitem{hw}
\BIBentryALTinterwordspacing
HuaWei, ``Huawei functiongraph,'' 2024, accessed 2024.05.30. [Online]. Available: \url{https://www.huaweicloud.com/product/functiongraph}
\BIBentrySTDinterwordspacing

\bibitem{aliwf}
\BIBentryALTinterwordspacing
Aliyun, ``Aliyun cloudflow,'' 2024, accessed 2024.05.30. [Online]. Available: \url{https://www.aliyun.com/product/aliware/fnf}
\BIBentrySTDinterwordspacing

\bibitem{awswf}
\BIBentryALTinterwordspacing
AWS, ``Aws step functions,'' 2024, accessed 2024.05.30. [Online]. Available: \url{https://aws.amazon.com/cn/step-functions}
\BIBentrySTDinterwordspacing

\bibitem{azwf}
\BIBentryALTinterwordspacing
Azure, ``Azure durable functions,'' 2024, accessed 2024.05.30. [Online]. Available: \url{https://learn.microsoft.com/en-us/azure/azure-functions/durable/durable-functions-overview?tabs=in-process%2Cnodejs-v3%2Cv1-model&pivots=csharp}
\BIBentrySTDinterwordspacing

\bibitem{serverlessbert}
\BIBentryALTinterwordspacing
P.~Schmid, ``serverless-bert-huggingface-aws-lambda-docker,'' 2024, accessed 2024.05.30. [Online]. Available: \url{https://github.com/philschmid/serverless-bert-huggingface-aws-lambda-docker}
\BIBentrySTDinterwordspacing

\bibitem{gwf}
\BIBentryALTinterwordspacing
Google, ``Google cloud composer,'' 2024, accessed 2024.05.30. [Online]. Available: \url{https://cloud.google.com/composer}
\BIBentrySTDinterwordspacing

\bibitem{docker}
\BIBentryALTinterwordspacing
Docker, ``The docker containerization platform,'' 2024, accessed 2024.05.30. [Online]. Available: \url{https://www.docker.com}
\BIBentrySTDinterwordspacing

\bibitem{agache2020firecracker}
A.~Agache, M.~Brooker, A.~Iordache, A.~Liguori, R.~Neugebauer, P.~Piwonka, and D.-M. Popa, ``Firecracker: Lightweight virtualization for serverless applications,'' in \emph{17th USENIX symposium on networked systems design and implementation (NSDI 20)}, 2020, pp. 419--434.

\bibitem{gviosr}
\BIBentryALTinterwordspacing
G.~gVisor, ``Google gvisor: Container runtime sandbox,'' 2024, accessed 2024.05.30. [Online]. Available: \url{https://github.com/google/gvisor}
\BIBentrySTDinterwordspacing

\bibitem{shahrad2020serverless}
M.~Shahrad, R.~Fonseca, I.~Goiri, G.~Chaudhry, P.~Batum, J.~Cooke, E.~Laureano, C.~Tresness, M.~Russinovich, and R.~Bianchini, ``Serverless in the wild: Characterizing and optimizing the serverless workload at a large cloud provider,'' in \emph{2020 USENIX Annual Technical Conference (USENIX ATC 20)}, 2020, pp. 205--218.

\bibitem{yang2022infless}
Y.~Yang, L.~Zhao, Y.~Li, H.~Zhang, J.~Li, M.~Zhao, X.~Chen, and K.~Li, ``Infless: a native serverless system for low-latency, high-throughput inference,'' in \emph{Proceedings of the 27th ACM International Conference on Architectural Support for Programming Languages and Operating Systems}, 2022, pp. 768--781.

\bibitem{scheuner2022let}
J.~Scheuner, S.~Eismann, S.~Talluri, E.~Van~Eyk, C.~Abad, P.~Leitner, and A.~Iosup, ``Let's trace it: Fine-grained serverless benchmarking using synchronous and asynchronous orchestrated applications,'' \emph{arXiv preprint arXiv:2205.07696}, 2022.

\bibitem{wang2017jointcloud}
H.~Wang, P.~Shi, and Y.~Zhang, ``Jointcloud: A cross-cloud cooperation architecture for integrated internet service customization,'' in \emph{2017 IEEE 37th international conference on distributed computing systems (ICDCS)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2017, pp. 1846--1855.

\bibitem{shi2019inherent}
P.~Shi, H.~Liu, S.~Yang, Y.~Zhang, and Y.~Zhong, ``The inherent mechanism and a case study of the constructional evolution of the jointcloud ecosystem,'' \emph{IEEE Internet of Things Journal}, vol.~7, no.~3, pp. 1561--1571, 2019.

\bibitem{safaryan2022slam}
G.~Safaryan, A.~Jindal, M.~Chadha, and M.~Gerndt, ``Slam: Slo-aware memory optimization for serverless applications,'' in \emph{2022 IEEE 15th International Conference on Cloud Computing (CLOUD)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2022, pp. 30--39.

\bibitem{wen2022stepconf}
Z.~Wen, Y.~Wang, and F.~Liu, ``Stepconf: Slo-aware dynamic resource configuration for serverless function workflows,'' in \emph{IEEE INFOCOM 2022-IEEE Conference on Computer Communications}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2022, pp. 1868--1877.

\bibitem{liu2020hcloud}
J.~Liu, Z.~Mi, Z.~Huang, Z.~Hua, and Y.~Xia, ``Hcloud: A serverless platform for jointcloud computing,'' in \emph{2020 IEEE International Conference on Joint Cloud Computing}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2020, pp. 86--93.

\bibitem{baarzi2021merits}
A.~F. Baarzi, G.~Kesidis, C.~Joe-Wong, and M.~Shahrad, ``On merits and viability of multi-cloud serverless,'' in \emph{Proceedings of the ACM Symposium on Cloud Computing}, 2021, pp. 600--608.

\bibitem{stoica2021cloud}
I.~Stoica and S.~Shenker, ``From cloud computing to sky computing,'' in \emph{Proceedings of the Workshop on Hot Topics in Operating Systems}, 2021, pp. 26--32.

\bibitem{maissen2020faasdom}
P.~Maissen, P.~Felber, P.~Kropf, and V.~Schiavoni, ``Faasdom: A benchmark suite for serverless computing,'' in \emph{Proceedings of the 14th ACM International Conference on Distributed and Event-based Systems}, 2020, pp. 73--84.

\bibitem{kim2019functionbench}
J.~Kim and K.~Lee, ``Functionbench: A suite of workloads for serverless cloud function service,'' in \emph{2019 IEEE 12th International Conference on Cloud Computing (CLOUD)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2019, pp. 502--504.

\bibitem{yu2020characterizing}
T.~Yu, Q.~Liu, D.~Du, Y.~Xia, B.~Zang, Z.~Lu, P.~Yang, C.~Qin, and H.~Chen, ``Characterizing serverless platforms with serverlessbench,'' in \emph{Proceedings of the 11th ACM Symposium on Cloud Computing}, 2020, pp. 30--44.

\bibitem{copik2021sebs}
M.~Copik, G.~Kwasniewski, M.~Besta, M.~Podstawski, and T.~Hoefler, ``Sebs: A serverless benchmark suite for function-as-a-service computing,'' in \emph{Proceedings of the 22nd International Middleware Conference}, 2021, pp. 64--78.

\bibitem{ristov2022faascinating}
S.~Ristov, D.~Kimovski, and T.~Fahringer, ``Faascinating resilience for serverless function choreographies in federated clouds,'' \emph{IEEE Transactions on Network and Service Management}, vol.~19, no.~3, pp. 2440--2452, 2022.

\bibitem{das2020skedulix}
A.~Das, A.~Leaf, C.~A. Varela, and S.~Patterson, ``Skedulix: Hybrid cloud scheduling for cost-efficient execution of serverless applications,'' in \emph{2020 IEEE 13th International Conference on Cloud Computing (CLOUD)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2020, pp. 609--618.

\bibitem{bao2019adaptive}
H.~Bao, Y.~Wang, and F.~Xu, ``An adaptive erasure code for jointcloud storage of internet of things big data,'' \emph{IEEE Internet of Things Journal}, vol.~7, no.~3, pp. 1613--1624, 2019.

\bibitem{ao2018sprocket}
L.~Ao, L.~Izhikevich, G.~M. Voelker, and G.~Porter, ``Sprocket: A serverless video processing framework,'' in \emph{Proceedings of the ACM Symposium on Cloud Computing}, 2018, pp. 263--274.

\bibitem{fouladi2017encoding}
S.~Fouladi, R.~S. Wahby, B.~Shacklett, K.~V. Balasubramaniam, W.~Zeng, R.~Bhalerao, A.~Sivaraman, G.~Porter, and K.~Winstein, ``Encoding, fast and slow:low-latency video processing using thousands of tiny threads,'' in \emph{14th USENIX Symposium on Networked Systems Design and Implementation (NSDI 17)}, 2017, pp. 363--376.

\bibitem{zhang2019mark}
C.~Zhang, M.~Yu, W.~Wang, and F.~Yan, ``Mark: Exploiting cloud services for cost-effective,slo-aware machine learning inference serving,'' in \emph{2019 USENIX Annual Technical Conference (USENIX ATC 19)}, 2019, pp. 1049--1062.

\bibitem{ali2020batch}
A.~Ali, R.~Pinciroli, F.~Yan, and E.~Smirni, ``Batch: machine learning inference serving on serverless platforms with adaptive batching,'' in \emph{SC20: International Conference for High Performance Computing, Networking, Storage and Analysis}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2020, pp. 1--15.

\bibitem{carreira2019cirrus}
J.~Carreira, P.~Fonseca, A.~Tumanov, A.~Zhang, and R.~Katz, ``Cirrus: A serverless framework for end-to-end ml workflows,'' in \emph{Proceedings of the ACM Symposium on Cloud Computing}, 2019, pp. 13--24.

\bibitem{thorpe2021dorylus}
J.~Thorpe, Y.~Qiao, J.~Eyolfson, S.~Teng, G.~Hu, Z.~Jia, J.~Wei, K.~Vora, R.~Netravali, M.~Kim \emph{et~al.}, ``Dorylus: Affordable, scalable, and accurate gnn training with distributed cpu servers and serverless threads,'' in \emph{15th USENIX Symposium on Operating Systems Design and Implementation (OSDI 21)}, 2021, pp. 495--514.

\bibitem{zhao2023beehive}
Z.~Zhao, M.~Wu, J.~Tang, B.~Zang, Z.~Wang, and H.~Chen, ``Beehive: Sub-second elasticity for web services with semi-faas execution,'' in \emph{Proceedings of the 28th ACM International Conference on Architectural Support for Programming Languages and Operating Systems, Volume 2}, 2023, pp. 74--87.

\bibitem{pu2019shuffling}
Q.~Pu, S.~Venkataraman, and I.~Stoica, ``Shuffling, fast and slow: Scalable analytics on serverless infrastructure,'' in \emph{16th USENIX symposium on networked systems design and implementation (NSDI 19)}, 2019, pp. 193--206.

\bibitem{jarachanthan2022astrea}
J.~Jarachanthan, L.~Chen, F.~Xu, and B.~Li, ``Astrea: Auto-serverless analytics towards cost-efficiency and qos-awareness,'' \emph{IEEE Transactions on Parallel and Distributed Systems}, vol.~33, no.~12, pp. 3833--3849, 2022.

\bibitem{fouladi2019laptop}
S.~Fouladi, F.~Romero, D.~Iter, Q.~Li, S.~Chatterjee, C.~Kozyrakis, M.~Zaharia, and K.~Winstein, ``From laptop to lambda: Outsourcing everyday jobs to thousands of transient functional containers,'' in \emph{2019 USENIX annual technical conference (USENIX ATC 19)}, 2019, pp. 475--488.

\bibitem{yang2023skypilot}
Z.~Yang, Z.~Wu, M.~Luo, W.-L. Chiang, R.~Bhardwaj, W.~Kwon, S.~Zhuang, F.~S. Luan, G.~Mittal, S.~Shenker \emph{et~al.}, ``Skypilot: An intercloud broker for sky computing,'' in \emph{20th USENIX Symposium on Networked Systems Design and Implementation (NSDI 23)}, 2023, pp. 437--455.

\bibitem{zhang2020kappa}
W.~Zhang, V.~Fang, A.~Panda, and S.~Shenker, ``Kappa: A programming framework for serverless computing,'' in \emph{Proceedings of the 11th ACM Symposium on Cloud Computing}, 2020, pp. 328--343.

\bibitem{khochare2023xfaas}
A.~Khochare, T.~Khare, V.~Kulkarni, and Y.~Simmhan, ``Xfaas: Cross-platform orchestration of faas workflows on hybrid clouds,'' in \emph{2023 IEEE/ACM 23rd International Symposium on Cluster, Cloud and Internet Computing (CCGrid)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2023, pp. 498--512.

\bibitem{wang2023edge}
Z.~Wang, S.~Zhang, J.~Cheng, Z.~Wu, Z.~Cao, and Y.~Cui, ``Edge-assisted adaptive configuration for serverless-based video analytics,'' in \emph{2023 IEEE 43rd International Conference on Distributed Computing Systems (ICDCS)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2023, pp. 248--258.

\bibitem{donkervliet2023servo}
J.~Donkervliet, J.~Ron, J.~Li, T.~Iancu, C.~L. Abad, and A.~Iosup, ``Servo: Increasing the scalability of modifiable virtual environments using serverless computing,'' in \emph{2023 IEEE 43rd International Conference on Distributed Computing Systems (ICDCS)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2023, pp. 829--840.

\bibitem{zhang2020fault}
H.~Zhang, A.~Cardoza, P.~B. Chen, S.~Angel, and V.~Liu, ``Fault-tolerant and transactional stateful serverless workflows,'' in \emph{14th USENIX Symposium on Operating Systems Design and Implementation (OSDI 20)}, 2020, pp. 1187--1204.

\bibitem{setty2016realizing}
S.~Setty, C.~Su, J.~R. Lorch, L.~Zhou, H.~Chen, P.~Patel, and J.~Ren, ``Realizing the $\{$Fault-Tolerance$\}$ promise of cloud storage using locks with intent,'' in \emph{12th USENIX Symposium on Operating Systems Design and Implementation (OSDI 16)}, 2016, pp. 501--516.

\bibitem{liu2023doing}
D.~H. Liu, A.~Levy, S.~Noghabi, and S.~Burckhardt, ``Doing more with less: Orchestrating serverless applications without an orchestrator,'' in \emph{20th USENIX Symposium on Networked Systems Design and Implementation (NSDI 23)}, 2023, pp. 1505--1519.

\bibitem{jia2021boki}
Z.~Jia and E.~Witchel, ``Boki: Stateful serverless computing with shared logs,'' in \emph{Proceedings of the ACM SIGOPS 28th Symposium on Operating Systems Principles}, 2021, pp. 691--707.

\bibitem{kenton2019bert}
J.~D. M.-W.~C. Kenton and L.~K. Toutanova, ``Bert: Pre-training of deep bidirectional transformers for language understanding,'' in \emph{Proceedings of NAACL-HLT}, 2019, pp. 4171--4186.

\bibitem{he2016deep}
K.~He, X.~Zhang, S.~Ren, and J.~Sun, ``Deep residual learning for image recognition,'' in \emph{Proceedings of the IEEE conference on computer vision and pattern recognition}, 2016, pp. 770--778.

\bibitem{jonas2017occupy}
E.~Jonas, Q.~Pu, S.~Venkataraman, I.~Stoica, and B.~Recht, ``Occupy the cloud: Distributed computing for the 99\%,'' in \emph{Proceedings of the 2017 Symposium on Cloud Computing (SOCC)}, 2017, pp. 445--451.

\bibitem{burckhardt2021durable}
S.~Burckhardt, C.~Gillum, D.~Justo, K.~Kallas, C.~McMahon, and C.~S. Meiklejohn, ``Durable functions: Semantics for stateful serverless,'' \emph{Proceedings of the ACM on Programming Languages}, vol.~5, no. OOPSLA, pp. 1--27, 2021.


\bibitem{mittal2021mu}
V.~Mittal, S.~Qi, R.~Bhattacharya, X.~Lyu, J.~Li, S.~G. Kulkarni, D.~Li, J.~Hwang, K.~Ramakrishnan, and T.~Wood, ``Mu: An efficient, fair and responsive serverless framework for resource-constrained edge clouds,'' in \emph{Proceedings of the ACM Symposium on Cloud Computing (SOCC)}, 2021, pp. 168--181.

\bibitem{liang2023edgeorcher}
Y.~Liang, Z.~Zhou, and X.~Chen, ``Edgeorcher: Predictive function orchestration for serverless-based edge native applications,'' in \emph{2023 IEEE 43rd International Conference on Distributed Computing Systems (ICDCS)}, 2023, pp. 1--2.

\bibitem{gadepalli2020sledge}
P.~K. Gadepalli, S.~McBride, G.~Peach, L.~Cherkasova, and G.~Parmer, ``Sledge: A serverless-first, light-weight wasm runtime for the edge,'' in \emph{Proceedings of the 21st International Middleware Conference (Middleware)}, 2020, pp. 265--279.

\bibitem{zhang2021edge}
M.~Zhang, C.~Krintz, and R.~Wolski, ``Edge-adaptable serverless acceleration for machine learning internet of things applications,'' \emph{Software: Practice and Experience}, vol.~51, no.~9, pp. 1852--1867, 2021.

\bibitem{xu2021lambdadnn}
F.~Xu, Y.~Qin, L.~Chen, Z.~Zhou, and F.~Liu, ``$\lambda$dnn: Achieving predictable distributed dnn training with serverless architectures,'' \emph{IEEE Transactions on Computers}, vol.~71, no.~2, pp. 450--463, 2021.

\bibitem{gu2023elasticflow}
D.~Gu, Y.~Zhao, Y.~Zhong, Y.~Xiong, Z.~Han, P.~Cheng, F.~Yang, G.~Huang, X.~Jin, and X.~Liu, ``Elasticflow: An elastic serverless training platform for distributed deep learning,'' in \emph{Proceedings of the 28th ACM International Conference on Architectural Support for Programming Languages and Operating Systems (ASPLOS)}, 2023, pp. 266--280.

\bibitem{joosen2023does}
A.~Joosen, A.~Hassan, M.~Asenov, R.~Singh, L.~Darlow, J.~Wang, and A.~Barker, ``How does it function? characterizing long-term trends in production serverless workloads,'' in \emph{Proceedings of the 2023 ACM Symposium on Cloud Computing (SOCC)}, 2023, pp. 443--458.

\bibitem{sreekanti20cloudburst}
V.~Sreekanti, C.~Wu, X.~C. Lin, J.~Schleier-Smith, J.~E. Gonzalez, J.~M. Hellerstein, and A.~Tumanov, ``Cloudburst: Stateful functions-as-a-service,'' \emph{Proceedings of the VLDB Endowment}, vol.~13, no.~11, pp. 2438--2452, 2020.

\bibitem{sreekanti2020fault}
V.~Sreekanti, C.~Wu, S.~Chhatrapati, J.~E. Gonzalez, J.~M. Hellerstein, and J.~M. Faleiro, ``A fault-tolerance shim for serverless computing,'' in \emph{Proceedings of the Fifteenth European Conference on Computer Systems (EuroSys)}, 2020, pp. 1--15.

\bibitem{klimovic2018pocket}
A.~Klimovic, Y.~Wang, P.~Stuedi, A.~Trivedi, J.~Pfefferle, and C.~Kozyrakis, ``Pocket: Elastic ephemeral storage for serverless analytics,'' in \emph{13th USENIX Symposium on Operating Systems Design and Implementation (OSDI 18)}, 2018, pp. 427--444.

\bibitem{shillaker2020faasm}
S.~Shillaker and P.~Pietzuch, ``Faasm: Lightweight isolation for efficient stateful serverless computing,'' in \emph{2020 USENIX Annual Technical Conference (USENIX ATC 20)}, 2020, pp. 419--433.

\bibitem{li2022faasflow}
Z.~Li, Y.~Liu, L.~Guo, Q.~Chen, J.~Cheng, W.~Zheng, and M.~Guo, ``Faasflow: Enable efficient workflow execution for function-as-a-service,'' in \emph{Proceedings of the 27th ACM International Conference on Architectural Support for Programming Languages and Operating Systems (ASPLOS)}, 2022, pp. 782--796.

\bibitem{carver2020wukong}
B.~Carver, J.~Zhang, A.~Wang, A.~Anwar, P.~Wu, and Y.~Cheng, ``Wukong: A scalable and locality-enhanced framework for serverless parallel computing,'' in \emph{Proceedings of the 11th ACM Symposium on Cloud Computing (SOCC)}, 2020, pp. 1--15.

\bibitem{malawski2020serverless}
M.~Malawski, A.~Gajek, A.~Zima, B.~Balis, and K.~Figiela, ``Serverless execution of scientific workflows: Experiments with hyperflow, aws lambda and google cloud functions,'' \emph{Future Generation Computer Systems}, vol. 110, no.~17, pp. 502--514, 2020.

\bibitem{shankar2020serverless}
V.~Shankar, K.~Krauth, K.~Vodrahalli, Q.~Pu, B.~Recht, I.~Stoica, J.~Ragan-Kelley, E.~Jonas, and S.~Venkataraman, ``Serverless linear algebra,'' in \emph{Proceedings of the 11th ACM Symposium on Cloud Computing (SOCC)}, 2020, pp. 281--295.

\bibitem{lopez2018comparison}
P.~G. L{\'o}pez, M.~S{\'a}nchez-Artigas, G.~Par{\'\i}s, D.~B. Pons, {\'A}.~R. Ollobarren, and D.~A. Pinto, ``Comparison of faas orchestration systems,'' in \emph{2018 IEEE/ACM International Conference on Utility and Cloud Computing Companion (UCC Companion)}, 2018, pp. 148--153.

\bibitem{jia2021nightcore}
Z.~Jia and E.~Witchel, ``Nightcore: efficient and scalable serverless computing for latency-sensitive, interactive microservices,'' in \emph{Proceedings of the 26th ACM International Conference on Architectural Support for Programming Languages and Operating Systems (ASPLOS)}, 2021, pp. 152--166.

\bibitem{mahgoub2021sonic}
A.~Mahgoub, L.~Wang, K.~Shankar, Y.~Zhang, H.~Tian, S.~Mitra, Y.~Peng, H.~Wang, A.~Klimovic, H.~Yang \emph{et~al.}, ``Sonic: Application-aware data passing for chained serverless applications,'' in \emph{2021 USENIX Annual Technical Conference (USENIX ATC 21)}, 2021, pp. 285--301.

\bibitem{kotni2021faastlane}
S.~Kotni, A.~Nayak, V.~Ganapathy, and A.~Basu, ``Faastlane: Accelerating function-as-a-service workflows,'' in \emph{2021 USENIX Annual Technical Conference (USENIX ATC 21)}, 2021, pp. 805--820.

\bibitem{bhasi2021kraken}
V.~M. Bhasi, J.~R. Gunasekaran, P.~Thinakaran, C.~S. Mishra, M.~T. Kandemir, and C.~Das, ``Kraken: Adaptive container provisioning for deploying dynamic dags in serverless platforms,'' in \emph{Proceedings of the ACM Symposium on Cloud Computing (SOCC)}, 2021, pp. 153--167.

\bibitem{burckhardt2022netherite}
S.~Burckhardt, B.~Chandramouli, C.~Gillum, D.~Justo, K.~Kallas, C.~McMahon, C.~S. Meiklejohn, and X.~Zhu, ``Netherite: Efficient execution of serverless workflows,'' \emph{Proceedings of the VLDB Endowment}, vol.~15, no.~8, pp. 1591--1604, 2022.

\bibitem{delimitrou2013paragon}
C.~Delimitrou and C.~Kozyrakis, ``Paragon: Qos-aware scheduling for heterogeneous datacenters,'' \emph{ACM SIGPLAN Notices}, vol.~48, no.~4, pp. 77--88, 2013.

\bibitem{delimitrou2014quasar}
------, ``Quasar: Resource-efficient and qos-aware cluster management,'' \emph{ACM SIGPLAN Notices}, vol.~49, no.~4, pp. 127--144, 2014.

\bibitem{gan2019seer}
Y.~Gan, Y.~Zhang, K.~Hu, D.~Cheng, Y.~He, M.~Pancholi, and C.~Delimitrou, ``Seer: Leveraging big data to navigate the complexity of performance debugging in cloud microservices,'' in \emph{Proceedings of the 24th ACM International Conference on Architectural Support for Programming Languages and Operating Systems (ASPLOS)}, 2019, pp. 19--33.

\bibitem{zhang2021sinan}
Y.~Zhang, W.~Hua, Z.~Zhou, G.~E. Suh, and C.~Delimitrou, ``Sinan: Ml-based and qos-aware resource management for cloud microservices,'' in \emph{Proceedings of the 26th ACM International Conference on Architectural Support for Programming Languages and Operating Systems (ASPLOS)}, 2021, pp. 167--181.

\bibitem{yang2013bubble}
H.~Yang, A.~Breslow, J.~Mars, and L.~Tang, ``Bubble-flux: Precise online qos management for increased utilization in warehouse scale computers,'' \emph{ACM SIGARCH Computer Architecture News}, vol.~41, no.~3, pp. 607--618, 2013.

\bibitem{zhou2022aquatope}
Z.~Zhou, Y.~Zhang, and C.~Delimitrou, ``Aquatope: Qos-and-uncertainty-aware resource management for multi-stage serverless workflows,'' in \emph{Proceedings of the 28th ACM International Conference on Architectural Support for Programming Languages and Operating Systems (ASPLOS)}, 2022, pp. 1--14.

\bibitem{lin2020modeling}
C.~Lin and H.~Khazaei, ``Modeling and optimization of performance and cost of serverless applications,'' \emph{IEEE Transactions on Parallel and Distributed Systems}, vol.~32, no.~3, pp. 615--632, 2020.

\bibitem{daw2020xanadu}
N.~Daw, U.~Bellur, and P.~Kulkarni, ``Xanadu: Mitigating cascading cold starts in serverless function chain deployments,'' in \emph{Proceedings of the 21st International Middleware Conferences (Middleware)}, 2020, pp. 356--370.

\bibitem{risco2021serverless}
S.~Risco, G.~Molt{\'o}, D.~M. Naranjo, and I.~Blanquer, ``Serverless workflows for containerised applications in the cloud continuum,'' \emph{Journal of Grid Computing}, vol.~19, no.~30, pp. 1--18, 2021.

\bibitem{mahgoub2022orion}
A.~Mahgoub, E.~B. Yi, K.~Shankar, S.~Elnikety, S.~Chaterji, and S.~Bagchi, ``Orion and the three rights: Sizing, bundling, and prewarming for serverless dags,'' in \emph{16th USENIX Symposium on Operating Systems Design and Implementation (OSDI 22)}, 2022, pp. 303--320.

\bibitem{mahgoub2022wisefuse}
A.~Mahgoub, E.~B. Yi, K.~Shankar, E.~Minocha, S.~Elnikety, S.~Bagchi, and S.~Chaterji, ``Wisefuse: Workload characterization and dag transformation for serverless workflows,'' \emph{Proceedings of the ACM on Measurement and Analysis of Computing Systems}, vol.~6, no.~2, pp. 1--28, 2022.

\bibitem{balis2016hyperflow}
B.~Balis, ``Hyperflow: A model of computation, programming approach and enactment engine for complex distributed workflows,'' \emph{Future Generation Computer Systems}, vol.~55, no.~1, pp. 147--162, 2016.

\bibitem{aske2018supporting}
A.~Aske and X.~Zhao, ``Supporting multi-provider serverless computing on the edge,'' in \emph{Workshop Proceedings of the 47th International Conference on Parallel Processing (ICPP Workshop)}, 2018, pp. 1--6.

\bibitem{perez2019premises}
A.~P{\'e}rez, S.~Risco, D.~M. Naranjo, M.~Caballer, and G.~Molt{\'o}, ``On-premises serverless computing for event-driven data processing applications,'' in \emph{2019 IEEE 12th International Conference on Cloud Computing (CLOUD)}, 2019, pp. 414--421.

\bibitem{perez2018serverless}
A.~P{\'e}rez, G.~Molt{\'o}, M.~Caballer, and A.~Calatrava, ``Serverless computing for container-based architectures,'' \emph{Future Generation Computer Systems}, vol.~83, no.~5, pp. 50--59, 2018.

\bibitem{smith2022fado}
C.~P. Smith, A.~Jindal, M.~Chadha, M.~Gerndt, and S.~Benedict, ``Fado: Faas functions and data orchestrator for multiple serverless edge-cloud clusters,'' in \emph{2022 IEEE 6th International conference on fog and edge computing (ICFEC)}, 2022, pp. 17--25.

\bibitem{ristov2022faast}
S.~Ristov and P.~Gritsch, ``Faast: Optimize makespan of serverless workflows in federated commercial faas,'' in \emph{2022 IEEE International Conference on Cluster Computing (CLUSTER)}, 2022, pp. 183--194.

\bibitem{jindal2021courier}
A.~Jindal, J.~Frielinghaus, M.~Chadha, and M.~Gerndt, ``Courier: Delivering serverless functions within heterogeneous faas deployments,'' in \emph{Proceedings of the 14th IEEE/ACM International Conference on Utility and Cloud Computing (UCC)}, 2021, pp. 1--10.

\bibitem{cordingly2023towards}
R.~Cordingly, J.~Kaur, D.~Dwivedi, and W.~Lloyd, ``Towards serverless sky computing: An investigation on global workload distribution to mitigate carbon intensity, network latency, and cost,'' in \emph{2023 IEEE International Conference on Cloud Engineering (IC2E)}, 2023, pp. 59--69.

\bibitem{chasins2022sky}
S.~Chasins, A.~Cheung, N.~Crooks, A.~Ghodsi, K.~Goldberg, J.~E. Gonzalez, J.~M. Hellerstein, M.~I. Jordan, A.~D. Joseph, M.~W. Mahoney \emph{et~al.}, ``The sky above the clouds,'' \emph{arXiv preprint arXiv:2205.07147}, 2022.

\bibitem{jain2023skyplane}
P.~Jain, S.~Kumar, S.~Wooders, S.~G. Patil, J.~E. Gonzalez, and I.~Stoica, ``Skyplane: Optimizing transfer cost and throughput using cloud-aware overlays,'' in \emph{20th USENIX Symposium on Networked Systems Design and Implementation (NSDI 23)}, 2023, pp. 1375--1389.

\bibitem{jia2015supercloud}
Q.~Jia, Z.~Shen, W.~Song, R.~Van~Renesse, and H.~Weatherspoon, ``Supercloud: Opportunities and challenges,'' \emph{ACM SIGOPS Operating Systems Review}, vol.~49, no.~1, pp. 137--141, 2015.

\bibitem{lu2013internet}
X.~Lu, H.~Wang, J.~Wang, J.~Xu, and D.~Li, ``Internet-based virtual computing environment: Beyond the data center as a computer,'' \emph{Future Generation Computer Systems}, vol.~29, no.~1, pp. 309--322, 2013.

\bibitem{wu2013spanstore}
Z.~Wu, M.~Butkiewicz, D.~Perkins, E.~Katz-Bassett, and H.~V. Madhyastha, ``Spanstore: Cost-effective geo-replicated storage spanning multiple cloud services,'' in \emph{Proceedings of the Twenty-Fourth ACM Symposium on Operating Systems Principles (SOSP)}, 2013, pp. 292--308.

\bibitem{wu2015costlo}
Z.~Wu, C.~Yu, and H.~V. Madhyastha, ``Costlo:cost-effective redundancy for lower latency variance on cloud storage services,'' in \emph{12th USENIX Symposium on Networked Systems Design and Implementation (NSDI 15)}, 2015, pp. 543--557.

\bibitem{pu2015low}
Q.~Pu, G.~Ananthanarayanan, P.~Bodik, S.~Kandula, A.~Akella, P.~Bahl, and I.~Stoica, ``Low latency geo-distributed data analytics,'' \emph{ACM SIGCOMM Computer Communication Review}, vol.~45, no.~4, pp. 421--434, 2015.

\bibitem{hung2018wide}
C.-C. Hung, G.~Ananthanarayanan, L.~Golubchik, M.~Yu, and M.~Zhang, ``Wide-area analytics with multiple resources,'' in \emph{Proceedings of the Thirteenth EuroSys Conference}, 2018, pp. 1--16.

\bibitem{weinman2015intercloudonomics}
J.~Weinman, ``Intercloudonomics: Quantifying the value of the intercloud,'' \emph{IEEE Cloud Computing}, vol.~2, no.~5, pp. 40--47, 2015.

\bibitem{eismann2021state}
S.~Eismann, J.~Scheuner, E.~Van~Eyk, M.~Schwinger, J.~Grohmann, N.~Herbst, C.~L. Abad, and A.~Iosup, ``The state of serverless applications: Collection, characterization, and community consensus,'' \emph{IEEE Transactions on Software Engineering}, vol.~48, no.~10, pp. 4152--4166, 2021.

\bibitem{gujarati2017swayam}
A.~Gujarati, S.~Elnikety, Y.~He, K.~S. McKinley, and B.~B. Brandenburg, ``Swayam: Distributed autoscaling to meet slas of machine learning inference services with resource efficiency,'' in \emph{Proceedings of the 18th ACM/IFIP/USENIX Middleware Conference (Middleware)}, 2017, pp. 109--120.

\bibitem{wen2021measurement}
J.~Wen and Y.~Liu, ``A measurement study on serverless workflow services,'' in \emph{2021 IEEE International Conference on Web Services (ICWS)}, 2021, pp. 741--750.

\bibitem{wen2023characterizing}
J.~Wen, Y.~Liu, Z.~Chen, J.~Chen, and Y.~Ma, ``Characterizing commodity serverless computing platforms,'' \emph{Journal of Software: Evolution and Process}, vol.~35, no.~10, pp. 2394--2417, 2023.

\bibitem{kim2019practical}
J.~Kim and K.~Lee, ``Practical cloud workloads for serverless faas,'' in \emph{Proceedings of the ACM Symposium on Cloud Computing (SOCC)}, 2019, pp. 477--477.

\bibitem{yu2023following}
M.~Yu, T.~Cao, W.~Wang, and R.~Chen, ``Following the data, not the function: Rethinking function orchestration in serverless computing,'' in \emph{20th USENIX Symposium on Networked Systems Design and Implementation (NSDI 23)}, 2023, pp. 1489--1504.

\bibitem{kijak2018challenges}
J.~Kijak, P.~Martyna, M.~Pawlik, B.~Balis, and M.~Malawski, ``Challenges for scheduling scientific workflows on cloud functions,'' in \emph{2018 IEEE 11th International Conference on Cloud Computing (CLOUD)}, 2018, pp. 460--467.

\bibitem{zhang2021caerus}
H.~Zhang, Y.~Tang, A.~Khandelwal, J.~Chen, and I.~Stoica, ``Caerus: Nimble task scheduling for serverless analytics,'' in \emph{18th USENIX Symposium on Networked Systems Design and Implementation (NSDI 21)}, 2021, pp. 653--669.

\bibitem{ghodsi2011dominant}
A.~Ghodsi, M.~Zaharia, B.~Hindman, A.~Konwinski, S.~Shenker, and I.~Stoica, ``Dominant resource fairness: Fair allocation of multiple resource types,'' in \emph{8th USENIX symposium on networked systems design and implementation (NSDI 11)}, 2011, p. 323–336.

\bibitem{grandl2014multi}
R.~Grandl, G.~Ananthanarayanan, S.~Kandula, S.~Rao, and A.~Akella, ``Multi-resource packing for cluster schedulers,'' \emph{ACM SIGCOMM Computer Communication Review}, vol.~44, no.~4, pp. 455--466, 2014.

\bibitem{grandl2016graphene}
R.~Grandl, S.~Kandula, S.~Rao, A.~Akella, and J.~Kulkarni, ``Graphene: Packing and dependency-aware scheduling for data-parallel clusters,'' in \emph{12th USENIX Symposium on Operating Systems Design and Implementation (OSDI 16)}, 2016, pp. 81--97.

\bibitem{grandl2016altruistic}
R.~Grandl, M.~Chowdhury, A.~Akella, and G.~Ananthanarayanan, ``Altruistic scheduling in multi-resource clusters,'' in \emph{12th USENIX Symposium on Operating Systems Design and Implementation (OSDI 16)}, 2016, pp. 65--80.

\bibitem{cordingly2020predicting}
R.~Cordingly, W.~Shu, and W.~J. Lloyd, ``Predicting performance and cost of serverless computing functions with saaf,'' in \emph{2020 IEEE Intl Conf on Dependable, Autonomic and Secure Computing, Intl Conf on Pervasive Intelligence and Computing, Intl Conf on Cloud and Big Data Computing, Intl Conf on Cyber Science and Technology Congress (DASC/PiCom/CBDCom/CyberSciTech)}, 2020, pp. 640--649.

\bibitem{eismann2021sizeless}
S.~Eismann, L.~Bui, J.~Grohmann, C.~Abad, N.~Herbst, and S.~Kounev, ``Sizeless: Predicting the optimal size of serverless functions,'' in \emph{Proceedings of the 22nd International Middleware Conference (Middleware)}, 2021, pp. 248--259.

\bibitem{gu2023time}
R.~Gu, X.~Chen, H.~Dai, S.~Wang, Z.~Wang, Y.~Tu, Y.~Huang, and G.~Chen, ``Time and cost-efficient cloud data transmission based on serverless computing compression,'' in \emph{IEEE INFOCOM 2023-IEEE Conference on Computer Communications (INFOCOM)}, 2023, pp. 1--10.

\bibitem{moghimi2023parrotfish}
A.~Moghimi, J.~Hattori, A.~Li, M.~Ben~Chikha, and M.~Shahrad, ``Parrotfish: Parametric regression for optimizing serverless functions,'' in \emph{Proceedings of the 2023 ACM Symposium on Cloud Computing (SOCC)}, 2023, pp. 177--192.

\bibitem{akhtar2020cose}
N.~Akhtar, A.~Raza, V.~Ishakian, and I.~Matta, ``Cose: Configuring serverless functions using statistical learning,'' in \emph{IEEE INFOCOM 2020-IEEE Conference on Computer Communications (INFOCOM)}, 2020, pp. 129--138.

\bibitem{zubko2022maff}
T.~Zubko, A.~Jindal, M.~Chadha, and M.~Gerndt, ``Maff: Self-adaptive memory optimization for serverless functions,'' in \emph{European Conference on Service-Oriented and Cloud Computing (ECOOP)}, 2022, pp. 137--154.

\bibitem{saha2018emars}
A.~Saha and S.~Jindal, ``Emars: Efficient management and allocation of resources in serverless,'' in \emph{2018 IEEE 11th International Conference on Cloud Computing (CLOUD)}, 2018, pp. 827--830.

\bibitem{ding2023automated}
H.~Ding, Z.~Wang, Z.~Shen, R.~Chen, and H.~Chen, ``Automated verification of idempotence for stateful serverless applications,'' in \emph{17th USENIX Symposium on Operating Systems Design and Implementation (OSDI 23)}, 2023, pp. 887--910.

\bibitem{elgamal2018costless}
T.~Elgamal, A.~Sandur, K.~Nahrstedt, and G.~Agha, ``Costless: Optimizing cost of serverless computing through function fusion and placement,'' in \emph{2018 IEEE/ACM Symposium on Edge Computing (SEC)}, 2018, pp. 300--312.

\bibitem{ristov2021xafcl}
S.~Ristov, S.~Pedratscher, and T.~Fahringer, ``Xafcl: Run scalable function choreographies across multiple faas systems,'' \emph{IEEE Transactions on Services Computing}, vol.~16, no.~1, pp. 711--723, 2021.

\bibitem{wang2018peeking}
L.~Wang, M.~Li, Y.~Zhang, T.~Ristenpart, and M.~Swift, ``Peeking behind the curtains of serverless platforms,'' in \emph{2018 USENIX Annual Technical Conference (USENIX ATC 18)}, 2018, pp. 133--146.

\bibitem{sampe2018serverless}
J.~Samp{\'e}, G.~Vernik, M.~S{\'a}nchez-Artigas, and P.~Garc{\'\i}a-L{\'o}pez, ``Serverless data analytics in the ibm cloud,'' in \emph{Proceedings of the 19th International Middleware Conference Industry}, 2018, pp. 1--8.

\bibitem{zheng2019globalflow}
G.~Zheng and Y.~Peng, ``Globalflow: A cross-region orchestration service for serverless computing services,'' in \emph{2019 IEEE 12th International Conference on Cloud Computing (CLOUD)}, 2019, pp. 508--510.

\bibitem{hellerstein2018serverless}
J.~M. Hellerstein, J.~Faleiro, J.~E. Gonzalez, J.~Schleier-Smith, V.~Sreekanti, A.~Tumanov, and C.~Wu, ``Serverless computing: One step forward, two steps back,'' \emph{arXiv preprint arXiv:1812.03651}, 2018.

\bibitem{du2022serverless}
D.~Du, Q.~Liu, X.~Jiang, Y.~Xia, B.~Zang, and H.~Chen, ``Serverless computing on heterogeneous computers,'' in \emph{Proceedings of the 27th ACM international conference on architectural support for programming languages and operating systems}, 2022, pp. 797--813.


\bibitem{devlin2018bert}
J.~Devlin, M.-W. Chang, K.~Lee, and K.~Toutanova, ``BERT: Pre-training of deep bidirectional transformers for language understanding,'' in \emph{Proceedings of the 2019 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 1 (Long and Short Papers)}, Minneapolis, Minnesota, 2019, pp. 4171–4186.
\bibitem{sanchez2020primula}
M.~S{\'a}nchez-Artigas, G.~T. Eizaguirre, G.~Vernik, L.~Stuart, and P.~Garc{\'\i}a-L{\'o}pez, ``Primula: A practical shuffle/sort operator for serverless computing,'' in \emph{Proceedings of the 21st International Middleware Conference Industrial Track}, 2020, pp. 31--37.

\end{thebibliography}
